NeuralUQ: A comprehensive library for uncertainty quantification in neural differential equations and operators

Uncertainty quantification (UQ) in machine learning is currently drawing increasing research interest, driven by the rapid deployment of deep neural networks across different fields, such as computer vision, natural language processing, and the need for reliable tools in risk-sensitive applications. Recently, various machine learning models have also been developed to tackle problems in the field of scientific computing with applications to computational science and engineering (CSE). Physics-informed neural networks and deep operator networks are two such models for solving partial differential equations and learning operator mappings, respectively. In this regard, a comprehensive study of UQ methods tailored specifically for scientific machine learning (SciML) models has been provided in [45]. Nevertheless, and despite their theoretical merit, implementations of these methods are not straightforward, especially in large-scale CSE applications, hindering their broad adoption in both research and industry settings. In this paper, we present an open-source Python library (https://github.com/Crunch-UQ4MI), termed NeuralUQ and accompanied by an educational tutorial, for employing UQ methods for SciML in a convenient and structured manner. The library, designed for both educational and research purposes, supports multiple modern UQ methods and SciML models. It is based on a succinct workflow and facilitates flexible employment and easy extensions by the users. We first present a tutorial of NeuralUQ and subsequently demonstrate its applicability and efficiency in four diverse examples, involving dynamical systems and high-dimensional parametric and time-dependent PDEs.

==> IN_introduction2.tex <==

Physics-informed and more generally scientific machine learning (SciML) provide potent tools for accurately modeling and predicting the dynamic response of physical systems; see \cite{karniadakis2021physicsinformed,cuomo2022scientific} for a comprehensive review as well as \cite{cai2022physics,psaros2022uncertainty}.
Neural network (NN) architectures for solving ordinary/partial differential equations (ODEs, PDEs), such as the physics-informed NN (PINN), and for learning operator mappings, such as the deep operator network (DeepONet), seamlessly combine scattered observational data with available physical models.
Specifically, they can address mixed
problems when only partial observational data and information regarding the underlying physical system
are available (e.g., \cite{raissi2020hidden,cai2021flow}); it is straightforward to incorporate noisy and multi-fidelity data (e.g., \cite{yang2021bpinns,meng2021learning,meng2020composite,meng2021multifidelity});
they can provide physically consistent predictions even for extrapolatory tasks (e.g., \cite{yang2021bpinns}); they do not
require computationally expensive mesh generation (e.g., \cite{raissi2019physicsinformed,lu2021deepxde}); and open-source software is available and
continuously extended (e.g., \cite{lu2021deepxde,chen2020neurodiffeq,haghighat2021sciann}). 
{\color{red} We refer to problems in which (1) the physics or ODE/PDEs are known as \textit{physics-informed learning} problems, and (2) the physics or ODE/PDEs are unknown or partially known as \textit{physics-agnostic learning} problems.}

However, uncertainty, associated with noisy and limited data as well as NN
overparametrization, for example, can degrade the accuracy of these models significantly \cite{abdar2021review,psaros2022uncertainty}.
As a result, uncertainty quantification (UQ) is paramount for deep learning to be \textit{reliably} used in critical applications involving
physical and biological systems \cite{wilson2020case}. 
In Fig.~\ref{fig:sciml_pie}, we provide an overview of SciML problems of interest as well as different sources of uncertainty.
In addition to reliability concerns, UQ is also necessary for efficient and economical design; for capital budgeting and risk-adaptive decision making in related projects; and even for assessing investment opportunities involving such systems in the form of real options \cite{richard2006real,de2008real}.
Clearly, this broad view of applications gives to UQ an additional dimension pertaining to the potential of \textit{harnessing uncertainty}, and renders it an indispensable research area of SciML applied to CSE problems and beyond.

%\begin{itemize}
% \item (super quantiles? http://faculty.nps.edu/joroyset/? Real options?)
% \item real options?
%\end{itemize}

Further, UQ in SciML is considerably more challenging than in traditional numerical solvers because of optimization-related issues of the over-parameterized neural networks, as well as the various uncertainties shown in Fig.~\ref{fig:sciml_pie}.
In addition, SciML is applied to increasingly more diverse problems, from steady to time-dependent and high-dimensional ones, and to problems involving systems given only in the form of black-box models (see, e.g., \cite{yang2021bpinns,meng2022learning,psaros2022uncertainty,han2018solving,darbon2020overcoming}).
Further, evaluating the performance of the available UQ methods is not straightforward, especially in situations involving limited data.
In this regard, Psaros et al. \cite{psaros2022uncertainty} provided an extensive review and proposed novel methods of UQ for SciML.
Nevertheless, employing current methods in large-scale applications and developing new ones, where trustworthy implementations and fast experimentation are needed, requires an up-to-date, well-maintained, and versatile software package.
To this end, we present in this paper an open-source Python library termed DeepXUQ, which can be accessed at: {\color{red} link in github}.
{\color{blue} {This paper can be viewed as complementary to, yet independent of, \cite{psaros2022uncertainty}.}}
We expect that DeepXUQ will be a useful toolbox for both practitioners and researchers, who either choose to apply off-the-shelf methods for solving their problems, or to build their own methods based on ones the library current supports. 
%We view DeepXUQ as a complement to \cite{psaros2022uncertainty} and we expect that it will be a useful toolbox for both practitioners and researchers, who either choose to apply off-the-shelf methods for solving their problems, or to build their own methods using our modular library.
In passing, we note that DeepXUQ is constantly updated and its most recent capabilities can be viewed in the GitHub repository.

We organize the paper as follows. 
In Section 2, we briefly present SciML as well as the PINN and DeepONet methods, which
are the building blocks of all the methods we discuss in this paper; however, other 
neural models for PDEs and operators can be employed as well. 
In Section 3, we describe the design of the DeepXUQ library, which includes model construction, posterior inference, and performance evaluation as well as post-training calibration.
In Section 4, we provide four computational examples for demonstrating the applicability and capabilities of our library.
Lastly, in Section 5, we conclude with the findings of this work and discuss future research.

\begin{figure}[!ht]
	\centering
	\includegraphics[width=0.95\linewidth]{./figs/SciML_Pie_Chart.png}
	\caption{\label{fig:sciml_pie}
	Schematic overview of a SciML problem scenario.
	As shown in (a), SciML problems of interest include, but are not limited to, forward, inverse and mixed ODEs/PDEs, and operator learning problems. 
	Next, in the pie chart of (b) a qualitative breakdown of total uncertainty is shown, describing the contributions from data (noisy, gappy); physical models (misspecification, stochasticity); neural networks (architecture, hyperparameters, overparametrization); and posterior inference. 
	Note that we mainly address two types of uncertainty in the current paper, i.e., aleatoric (data noise) and  epistemic (NN overparametrization and limited data) uncertainties. 
	As shown in (c), with the predicted uncertainty active learning for enhancing the predicted accuracy can be performed, i.e., acquire new inputs according to a certain acquisition function in the training dataset.  
}
\end{figure}




==> IN_library.tex <==
In this section, we first present an overview of the DeepXUQ library, and subsequently provide details regarding its design, use, and customization for extended capabilities. 
In passing, note that a distinct \texttt{font} is used for referring to the library modules in the text, with the respective bold \textbf{\texttt{font}} used only for referring to them for the first time in the main text.
Further, for each example module named \texttt{module}, multiple of its sub-modules named, e.g., \texttt{module.sub1} and \texttt{module.sub2}, are referred to in the text as \texttt{module.sub1}, \texttt{sub2}, for convenience.

\subsection{Library design overview}

\textcolor{red}{}

The value of $u$ at a location $x$ given the data $\cD$ is a random variable denoted by $(u|x, \cD)$.
The aim of UQ is to obtain samples from the posterior distribution $p(u|\pazocal{D})$.
To that end, in the design phase a model is constructed that includes surrogates representing the solution $u$ and potentially $f$ and/or $\lambda$; as well as likelihood functions representing the data distribution.
Surrogates are parametrized by $\theta$ and when combined with prior probability distributions of $\theta$ result to stochastic processes; i.e., a proposed family of solutions.
To select the solution function samples that best explain the data, a posterior inference method is combined with the model. 
Finally, the obtained function samples can be calibrated using additional data. In the revision phase, metrics are used for evaluating the performance and re-designing the solution procedure. 

\begin{algorithm}[htbp]
\caption{Usage of UQ4SciML for solving differential equations.}
\label{alg:uq4sciml}
\begin{enumerate}
\item[Step 1] Specify the surrogate for the solution to a differential equation using the \textbf{\texttt{process}} module.
\item[Step 2] Specify the differential equation using the automatic differentiation.
\item[Step 3] Construct the likelihoods or loss functions based on the equations, boundary/initial conditions, and or given data, using the \textbf{\texttt{losses}} module.
\item[Step 4] Combine the process and likelihoods/loss functions to construct a \textbf{\texttt{model}}.
\item[Step 5] Specify the inference method using the \textbf{\texttt{inference}} module.
\item[Step 6] Call \textbf{\texttt{model.compile}} for initialization of the hyperparameters, such as initial values for weights/biased in HMC, optimizer and learning rate, etc.
\item[Step 7] Call \textbf{\texttt{model.run}} to train the network to obtain the optimal hyperparameters. 
\item[Step 8] Feed the hyperparameters obtained at Step 7 to the surrogate from Step 1 to get the predicted function samples.
\end{enumerate}
\end{algorithm}


In this regard, the library comprises the respective components, as depicted in Fig.~\ref{fig:lib:overview}; i.e., the processes and likelihoods components that are used for constructing the model (Section~\ref{sec:model}), the inference component (Section~\ref{sec:inference}), as well as the calibration component (Section~\ref{sec:calibration}). The workflow for the present library is shown in Procedure \ref{alg:uq4sciml}. 

\begin{figure}[!ht]
	\centering
	\includegraphics[width=.9\linewidth]{./figs/design1.png}
	\caption{Library design overview.
	In the design phase, a model is constructed that includes processes representing a proposed solution family and likelihood or loss functions representing the data distribution.
	Processes include surrogates, which can be construed as assumed functional forms, and priors distributions or variables for the parameters of the surrogates, depending on the type of method used.
    Likelihoods or loss functions are constructed using the data and the underlying neural ODE/PDE.
    To select the solution function samples that best explain the data, a posterior inference method is combined with the model.
    Finally, the obtained function samples can be calibrated using additional data. 
    In the revision phase, metrics are used for evaluating the performance and re-designing the solution procedure.
	}
	\label{fig:lib:overview}
\end{figure}


\subsection{Model construction}\label{sec:model}

The model component of the library includes the processes and likelihoods components, which are described in the following.

\subsubsection{Process}\label{sec:processes}


% {\color{red} surrogate.bnn/fnn/gan}


For neural ODEs/PDEs, the solution $u$ is modeled with a \textit{surrogate} parametrized by $\theta$, i.e., $\cM$ in Fig.~\ref{fig:neurals}. {\color{red} In particular, the built-in primitive surrogates in UQ4SciML include \textbf{\texttt{surrogates.fnn}} (standard NNs), \textbf{\texttt{surrogates.bnn}} (BNNs), and \textbf{\texttt{surrogates.generator}} (GAN-based functional priors)}. These models are referred to as U-PINN, B-PINN and PI-GAN-FP, respectively, in \cite{psaros2022uncertainty}. 
In all cases different $\theta$ values correspond to different functions $u_{\theta}$. 
We refer to the surrogate combined with a probability distribution $p(\theta)$ for $\theta$ as a \textit{process}. 
As explained in Section~\ref{sec:inference}, posterior inference obtains representative $\theta$ samples that explain the data $\cD$, based on the process definition.
Also, the problem parameters $\lambda$ {\color{red} can either be unknown constants or unknown fields depending on the problem setup.}  {\color{red} In UQ4SciML, we employ  \textbf{\texttt{surrogates.identity}} and  \textbf{\texttt{surrogates.fnn/bnn/generator}} as the surrogate for the unknown constant and field, respectively. In particular, we parameterize the surrogates with $\theta_{\lambda}$. Further, posterior inference is performed for $\theta$ and $\theta_{\lambda}$ together}.

For the special case of learning neural operators described in Section~\ref{sec:sciml}, the solution $u$ is modeled with a DeepONet surrogate parametrized by $\theta$ and posterior inference is performed as above. 
This model is referred to as U-DeepONet in \cite{psaros2022uncertainty}.
However, for the more general case in which the inference input data are noisy, the DeepONet is pre-trained with fixed parameters, and the input $f$ is modeled with a BNN or a GAN-FP, denoted by $\cM$ in Fig.~\ref{fig:neurals}.
These models are referred to as PA-BNN-FP and PA-GAN-FP, respectively, in \cite{psaros2022uncertainty}. 
Posterior inference is performed as above for the BNN parameters $\theta$ or the GAN input $\theta$. {\color{red} In UQ4SciML, we utilize \textbf{\texttt{surrogate.deeponet}} and \textbf{\texttt{surrogate.generator}} for the implementations of U-DeepONet and PA-BNN-FP/PA-GAN-FP, respectively.}

In passing, note that the ensemble posterior inference methods, summarized in Table~\ref{tab:uqt:over}, do not require a prior $p(\theta)$ and thus, we only need to define the surrogate component.


\begin{figure}[!ht]
	\centering
	\includegraphics[width=.9\linewidth]{./figs/functional_prior.png}
	\caption{Surrogates employed for learning neural ODEs/PDEs and operators.
	For neural ODEs/PDEs, the solution $u$ is modeled with a surrogate parametrized by $\theta$. 
The surrogate $\cM$ can be a standard NN or a pre-trained GAN functional prior.
These models are referred to as U-PINN and PI-GAN-FP, respectively, in \cite{psaros2022uncertainty}.
In both cases different $\theta$ values correspond to different functions $u_{\theta}$. 
For the special case of learning neural operators described in Section~\ref{sec:sciml}, the solution $u$ is modeled with a DeepONet surrogate parametrized by $\theta$ and posterior inference is performed as above. 
This model is referred to as U-DeepONet in \cite{psaros2022uncertainty}.
For the more general case in which the inference input data are noisy, the DeepONet is pre-trained with fixed parameters, and the input $f$ is modeled with a BNN or a GAN-FP, denoted by $\cM$.
These models are referred to as PA-BNN-FP and PA-GAN-FP, respectively, in \cite{psaros2022uncertainty}.}
	\label{fig:neurals}
\end{figure}

\begin{figure}[!ht]
	\centering
	\includegraphics[width=.9\linewidth]{./figs/design2.png}
	\caption{Processes component (ZZ).}
\end{figure}

\subsubsection{Likelihoods}\label{sec:likelihoods}

Given a set of paired noisy observations $\cD = \{x_i,u_i\}_{i=1}^{N}$, our goal is to construct a distribution $p(u|x, \cD)$ for predicting the value of $u$ at any new location $x$. 
For each $x$, it is commonly assumed that $u(x)$ produced by the data-generating process contains both a deterministic part $u_c(x)$ as well as some additive noise $\epsilon_u$, i.e., $u(x) = u_c(x) + \epsilon_u$.
This noise is typically called data or aleatoric uncertainty. 
For modeling this process, we assume a \textit{likelihood function} denoted by $p(u|x, \theta)$, with parameters $\theta=[\theta_1,\dots,\theta_K]^T$ to be inferred from the available data.
Further, for defining $p(u|x, \theta)$ we construct a model $u_{\theta}(x)$ that captures the deterministic part of $u(x)$ at some location $x$ and assume a model for the noise.
For example, the factorized Gaussian likelihood function, given as
\begin{equation}\label{eq:uqt:pre:bma:Glike}
	p(u|x, \theta) = \cN(u|u_{\theta}(x), diag(\Sigma_{u}^2)) = \prod_{d = 1}^{D_u}\frac{1}{\sqrt{2\pi \sigma_{u}^2}}\exp(-\frac{(u_d-u_{\theta}(x)_d)^2}{2\sigma_{u}^2}), 
\end{equation}
with the subscript $d$ denoting each of the $D_u$ dimensions of $u$, is often used for multi-dimensional function approximation problems.
In Eq.~\eqref{eq:uqt:pre:bma:Glike}, the output vector $u_{\theta}(x)$ is the mean of the Gaussian distribution assumed for $u$ at location $x$, $diag(\Sigma_{u}^2)$ is a diagonal covariance matrix with $\Sigma_{u}^2 = [\sigma_{u}^2,\dots,\sigma_{u}^2]$ in the diagonal, and $\sigma_{u}^2$ may either be known or assumed, or inferred from data.

For neural ODEs/PDEs, the observations in the dataset $\cD = \{\cD_f, \cD_b, \cD_u, \cD_{\lambda}\}$ are typically obtained with a data acquisition device and are noisy. 
In this regard, we employ four likelihood functions for approximating the $f, b, u$ and $\lambda$ distributions, denoted as $p(f|x, \theta), p(b|x, \theta), p(u|x, \theta)$, and $p(\lambda|x, \theta)$, respectively.
The total likelihood of the dataset $\cD$ becomes
\begin{equation}\label{eq:uqt:pre:pinn:like}
	p(\cD|\theta) = p(\cD_f|\theta)p(\cD_b|\theta)p(\cD_{u}|\theta)p(\cD_{\lambda}|\theta),
\end{equation}
where 
\begin{equation}
\begin{aligned}\label{eq:uqt:pre:pinn:likes}
	p(\cD_f|\theta) & = \prod_{i=1}^{N_f}p(f_i|x_i, \theta) \text{; } & p(\cD_b|\theta) & = \prod_{i=1}^{N_b}p(b_i|x_i, \theta);\\
	p(\cD_u|\theta) & = \prod_{i=1}^{N_u}p(u_i|x_i, \theta) \text{; } & p(\cD_{\lambda}|\theta) & = \prod_{i=1}^{N_{\lambda}}p(\lambda_i|x_i, \theta).
\end{aligned}
\end{equation}

For neural operators, we assume that $f$ and $b$ in Eq.~\eqref{eq:intro:piml:pinn:pde} are known and the dataset $\cD_{\lambda}$ consists of clean data.
Nevertheless, $\cD_u$ consists of noisy data in general.
In this regard, a likelihood function is employed for the $u$ data, denoted by $p(u|x, \xi, \theta)$, and the total likelihood is given as
\begin{equation}\label{eq:uqt:pre:don:like}
    p(\cD|\theta) =\prod_{i=1}^{N}\prod_{j=1}^{N_u}p(u_j^{(i)}|x_j^{(i)}, \xi_i, \theta). 
\end{equation}

\subsection{Posterior inference}\label{sec:inference}

Performing UQ for neural ODEs/PDEs and operators involves combining the constructed model with a posterior inference method. 
In this section, we provide a summary of the considered method and describe the library components for producing surrogate parameter $\theta$ samples and subsequently, the sought function samples.

\subsubsection{Methods}\label{sec:inference:methods}

Obtaining the posterior distribution of $\theta$ is computationally and analytically intractable. 
To address this issue, approximate inference aims to approximate the posterior by another distribution and/or obtaining  NN parameter posterior samples $\{\hat{\theta}_j\}_{j=1}^M$ from the posterior.
In Table~\ref{tab:uqt:over} we provide an overview of the most commonly used methods for obtaining $\{\hat{\theta}_j\}_{j=1}^M$; see Fig.~\ref{tab:uqt:over} and \cite{psaros2022uncertainty} for more details.
We refer to the HMC, LD, MFVI, and LA methods as \textit{Bayesian}, because they are related with the Bayesian paradigm of obtaining posterior samples, and to the MCD, DEns, SEns, and SWAG methods as \textit{deterministic}, because they can be interpreted as extensions of standard, i.e, deterministic, training of NNs.
In the package, the default option is to combine the methods with a Bayesian neural network, as a surrogate.
Alternatively, a GAN functional prior can be used.

\textcolor{blue}{
UQ4SciML supports three different types of posterior estimation methods, i.e., sampling-based method, vi-based method, and . Specifically, the sampling- and vi-based posterior estimations are for \textit{Bayesian} methods, and the .  MCMC-based methods utilize Markov chain Monte Carlo to sample directly against, probably un-normalized, posterior distribution. We describe MCMC-based methods as sampling methods. Ensemble-based methods execute standard training of NNs, throughout which samples are collected to group an ensemble. We describe such methods as sampling-through-optimization ones. Finally, VI-based methods are closely related with variational inferences, where posterior is approximated by optimizing some distance, e.g. KL-divergence, between the real one and a parameterized one. After the optimization completes, samples are obtained by sampling against the trained parameterized distribution, and hence we describe such methods as optimizing-and-sampling ones. Types of inference methods should be consistent with the type of model, e.g. an MCMC-based method can not work with a variational inference model, even though they both belong to the family of Bayesian inference. More details will be discussed in (Section~\ref{sec:advanced}).
}

% \textcolor{blue}{We categorize inference methods into three classes, MCMC-based, ensemble-based and VI-based. MCMC-based methods utilize Markov chain Monte Carlo to sample directly against, probably un-normalized, posterior distribution. We describe MCMC-based methods as sampling methods. Ensemble-based methods execute standard training of NNs, throughout which samples are collected to group an ensemble. We describe such methods as sampling-through-optimization ones. Finally, VI-based methods are closely related with variational inferences, where posterior is approximated by optimizing some distance, e.g. KL-divergence, between the real one and a parameterized one. After the optimization completes, samples are obtained by sampling against the trained parameterized distribution, and hence we describe such methods as optimizing-and-sampling ones. Types of inference methods should be consistent with the type of model, e.g. an MCMC-based method can not work with a variational inference model, even though they both belong to the family of Bayesian inference. More details will be discussed in (Section~\ref{sec:advanced}).}

\textcolor{blue}{Remarks by ZZ:} % to be deleted
% remarks start
For current library, SEns, LA, SWAG are not implemented.
% remarks end

\begin{table}
	\centering
	\footnotesize
	\begin{tabular}{rcl}
		\toprule
		\multicolumn{3}{c}{\textbf{Methods for obtaining NN parameter posterior samples} $\{\hat{\theta}_j\}_{j=1}^M$} \\
		\midrule
		Method full name & Method & Short description
		\\
		\midrule
		Hamiltonian  &\multirow{2}{*}{HMC} &  Two-step MCMC \\
		Monte Carlo && (simulates Hamiltonian dynamics)  \\
		\arrayrulecolor{black!30}\midrule
		\multirow{2}{*}{Langevin dynamics} & \multirow{2}{*}{LD} &  One-step MCMC (stochastic gradient \\ && descent with added noise) \\
		\arrayrulecolor{black!30}\midrule
		Mean-field  & \multirow{2}{*}{MFVI} & Approximates $p(\theta|\cD)$ by a Gaussian \\variational inference&& variational distribution $q_{\omega}(\theta)$\\ 
		\arrayrulecolor{black!30}\midrule
		Monte Carlo  & \multirow{2}{*}{MCD} & Standard training with some \\dropout&& NN parameters set to zero in each step\\
		\arrayrulecolor{black!30}\midrule
		Laplace & \multirow{2}{*}{LA} &Standard training with a Gaussian \\approximation&& fitted to the discovered mode $\hat{\theta}$\\
		\arrayrulecolor{black!30}\midrule
		\multirow{2}{*}{Deep ensemble} & \multirow{2}{*}{DEns} & Standard training \\ && $M$ independent times \\
		\arrayrulecolor{black!30}\midrule
		\multirow{2}{*}{Snapshot ensemble} & \multirow{2}{*}{SEns} &  Snapshots during standard training \\ && with learning rate schedule \\
		\arrayrulecolor{black!30}\midrule
		Stochastic weight & \multirow{2}{*}{SWAG} & SEns with a Gaussian distribution \\averaging-Gaussian && fitted to the snapshots \\
		\arrayrulecolor{black!30}\midrule
		X with Bayesian & \multirow{2}{*}{X+BNN} & Combines above methods with a BNN \\neural network && \textit{(Default setting)}\\
		\arrayrulecolor{black!30}\midrule
		X with GAN & \multirow{2}{*}{X+FP} & Combines above methods with \\functional prior && GAN functional prior instead of BNN \\
		\arrayrulecolor{black}
		\bottomrule
	\end{tabular}
	\caption{Overview of the most commonly used methods for obtaining the parameter samples $\{\hat{\theta}_j\}_{j=1}^M$; see \cite{psaros2022uncertainty} for more details.
We refer to the HMC, LD, MFVI, and LA methods as \textit{Bayesian}, because they are related with the Bayesian paradigm of obtaining posterior samples, and to the MCD, DEns, SEns, and SWAG methods as \textit{deterministic}, because they can be interpreted as extensions of standard, i.e, deterministic, training of NNs.
In the package, the default option is to combine the methods with a Bayesian neural network, as a surrogate.
Alternatively, a GAN functional prior can be used.
	}
	\label{tab:uqt:over}
\end{table}

\subsubsection{From parameter to function samples}\label{sec:fsamples}

The value of $u$ at a location $x$ given the data $\cD$ is a random variable denoted by $(u|x, \cD)$.
The mean of $(u|x, \cD)$ is denoted by $\hat{u}(x) = \mathbb{E}[u|x, \cD]$ and approximated by $\bar{\mu}(x)$ as
\begin{equation}\label{eq:uqt:pre:mcestmc:mean}
	\hat{u}(x) \approx \bar{\mu}(x) = \frac{1}{M}\sum_{j=1}^Mu_{\hat{\theta}_j}(x),
\end{equation}
where $\{u_{\hat{\theta}_j}(x)\}_{j=1}^M$ is the set of NN predictions corresponding to the samples $\{\hat{\theta}_j\}_{j=1}^M$.
Further, the diagonal part of the covariance matrix of $(u|x, \cD)$ is given by
\begin{equation}\label{eq:uqt:pre:mcestmc:totvar}
	Var(u|x, \cD) \approx \bar{\sigma}^2(x) =  \underbrace{\Sigma_{u}^2}_{\bar{\sigma}_a^2(x)}  + \underbrace{\frac{1}{M}\sum_{j=1}^M(u_{\hat{\theta}_j}(x)-\bar{\mu}(x))^2}_{\bar{\sigma}_e^2(x)}. 
\end{equation} 
In this equation, $\bar{\sigma}^2(x)$ represents the approximate total uncertainty of $(u|x, \cD)$, while $\bar{\sigma}_a^2(x)$ and $\bar{\sigma}_e^2(x)$ denote the aleatoric and the epistemic parts of the total uncertainty, respectively.
In practice, a Gaussian (or, e.g., Student-t) distribution is commonly fitted to the posterior samples and used for both PDF and CDF evaluations.
For example, we denote as $\pazocal{N}(\bar{\mu}(x), \bar{\sigma}^2(x))$ the Gaussian approximation to the samples $\{u_{\hat{\theta}_j}(x)\}_{j=1}^M$ at an arbitrary location $x$, where $\bar{\mu}(x)$ and $\bar{\sigma}^2(x)$ are obtained via Eqs.~\eqref{eq:uqt:pre:mcestmc:mean} and \eqref{eq:uqt:pre:mcestmc:totvar}, respectively.

\subsection{Performance evaluation and post-training calibration}\label{sec:calibration}

In \cite{psaros2022uncertainty}, the authors present various metrics for performance evaluation using a test dataset, such as relative $\ell_2$ error for evaluating accuracy, mean predictive likelihood for evaluating predictive capacity, and root mean squared calibration error for evaluating statistical consistency; i.e., how closely the predictive model matches the data-generating distribution.
These are implemented in the metrics component of the library.

For post-training calibration, suppose that an additional dataset $\cD_r = \{x_i, u_i\}_{i=1}^{N_r}$ is available after training.
This can be a left-out calibration dataset, similar to validation and test sets.
In Table~\ref{tab:calibration}, we summarize three approaches for improving the calibration of function approximation predictive models after training, using the calibration dataset. 

\begin{table}
	\centering
	\footnotesize
	\begin{tabular}{clc}
		\toprule
		\multicolumn{3}{c}{\textbf{Post-training calibration methods}}\\
		\midrule
		Reference & Short description & Name in library
		\\
		\midrule
		\multirow{2}{*}{\cite{levi2019evaluating}}  &  Re-weighting optimally all predicted variances & \multirow{2}{*}{\textit{calibration.xxx}} \\
		 & Modifies only the variance of the predictions. & \\
		\arrayrulecolor{black!30}\midrule
		\multirow{3}{*}{\cite{kuleshov2018accurate}} &  Approximates misscalibration function & \multirow{3}{*}{\textit{calibration.xxx}}
		\\ & and applies it to all predictive distributions. &
         \\ & Modifies both the mean and the variance of all predictions. &\\
		\arrayrulecolor{black!30}\midrule
		\multirow{3}{*}{\cite{zelikman2020crude}} & An empirical distribution is fitted to the scaled residuals & \multirow{3}{*}{\textit{calibration.xxx}}
		\\ & that correspond to the calibration dataset.&
		\\& Modifies both the mean and the variance of all predictions.& \\ 
		\arrayrulecolor{black}
		\bottomrule
	\end{tabular}
	\caption{Overview of the post-training calibration methods considered in this paper (AP).
	}
	\label{tab:calibration}
\end{table}

\subsection{Advanced research and development}\label{sec:advanced}

In this section, we discuss advanced topics of our library. Besides direct applications, some of which are shown in section 4, the library also supports further modification and customization, e.g. customized prior distributions, surrogates, etc. In this paper, we mainly focus on developments upon variable, surrogate and inference method modules of the library. Further, we also cover synthesis of existing functionalities for more applications. Pseudo-codes and results are shown in appendix. Codes, details and examples can be found in the GitHub page.

\subsubsection{Customized variables}

There are in total three types of variables we consider in UQ4SciML, Trainable, Samplable and VI. Trainable stands for deterministic variables that are constants and capable of being trained or optimized, commonly seen in many non-UQ deep learning libraries these day. Samplable, on the other hand, stands for random variables that are capable of being sampled, whose posterior inference is obtained by using sampling methods, e.g. MCMC methods. Variables with this type are not able to be trained or optimized, and are not able to be traced implicitly by most libraries. VI stands for random variables with parameterized distributions, commonly seen in variational inference problems. VI variables are still able to be sampled. However, unlike Samplable variables, their posterior inference is done by approximating the posterior distribution through optimizing against some metrics, e.g. ELBO.

Variables with each type have different setups. For example, when Bayesian neural networks are deployed for function approximation with uncertainty, independent standard Normal prior distributions are generally used for all weights and biases, which corresponds to L2 regularization in deterministic frameworks. However, different prior distributions or regularization methods, e.g. Laplace distribution (L1 regularization), are more reasonable and meaningful than the other under certain circumstances. 

\subsubsection{Customized surrogates}

\subsubsection{Customized inference methods}

\subsubsection{Synthesis of existing functionalities}



\textcolor{red}{For example, OOD.}

\subsubsection{Scenario: developing new functionalities}


\textcolor{red}{For example, Laplace distribution for the prior distributions, different methods to obtain posterior samples.}


==> IN_library2.tex <==
\subsection{Library design overview}\label{sec:overview}


{\color{blue} {Target of this subsection: discuss and explain why and how we decompose UQ in SciML and form the general framework in Fig 2.}}

{\color{blue} {The first paragraph describes from where surrogate in Fig 2 comes (why we need surrogate).}}

The general purpose of this paper and the library is to obtain, quantify, calibrate and analyze uncertainty with, probably noisy, measurements and physics for different problems. Specifically, we are interested in estimating $p(u|x, \cD)$, which is the posterior distribution of a function, $u$, at any given location, $x$, given some measurements, $\cD$. However, most of times $u$ is of infinite dimensions, and in practice, we use a function parameterized by unknown $\theta$ in space of finite dimensions to approximate $u$. This function is generally referred as the surrogate, denoted by $u_\theta$, and $\theta$ is referred as its parameter(s).

{\color{blue} {The second paragraph describes how we obtain posterior distribution, from where likelihood and prior in Fig 2 come, and why they are important.}}

With the surrogate, estimating $p(u|x, \cD)$ now becomes estimating $p(\theta|\cD)$. It follows the Bayes' theorem that $p(\theta|\cD) = \frac{p(\cD|\theta)p(\theta)}{p(\cD)}$, where $p(\theta)$ is referred as the prior distribution of $\theta$ and $p(\cD|\theta)$ is referred as the likelihood distribution over $\cD$. The prior distribution is generally chosen such that through surrogate, $u_\theta$ matches the prior information over $u$, e.g. non-negativity, a Dirichlet boundary condition, and the likelihood distribution connects $\theta$ and $\cD$ by the surrogate and a properly chosen distribution, e.g. Gaussian distribution for regression problems, Bernoulli distribution for classification problems. In most problems, logarithm of the posterior distribution is considered, i.e. $\log p(\theta|\cD) = \log p(\theta) + \log p(\cD|\theta) - p(\cD)$.

{\color{blue} {The third paragraph describes why inference methods are needed, how we evaluate the distribution of $u$, and from where parameter samples and function sample come from.}}

Posterior, however, is generally analytically intractable. The intractability comes from $p(\cD) = \int p(\cD|\theta)p(\theta) d\theta$. That is, even though the prior and the likelihood distributions are known, $p(\cD)$ is hard to compute analytically. Exception happens when both the prior and the likelihood distributions are Gaussian. For that case, the posterior is another Gaussian, and the model becomes the well-known Gaussian Process regression ({\color{blue}{cite some GP papers here}}). To maintain high expressivity of the surrogate as well as the capability to tackle nonlinear problems, complicated surrogates are used and hence the likelihood distribution is generally not Gaussian, which indicates that, even though for the distribution of $\theta$ is analytical, e.g. the prior distribution, $u_\theta$ is not intractable because of the complicacy of the surrogate. Nevertheless, distributions of $\theta$ and $u_\theta$ are most commonly analyzed through their samples, and to obtain the samples, inference methods are used. Details about the inference methods will be discussed later {\color{blue}{refer the section here}}.

{\color{blue} {The fourth paragraph describes what a process is and how it integrates surrogate and distribution.}}

Together with its parameter $\theta$, a surrogate defines a function. In this paper, $\theta$ is in fact random and hence $u_\theta$ becomes a stochastic function/process, whose randomness is represented ({\color{blue} {another word?}}) with samples. The library refers such functions as \textit{processes}. Generally, each process comes with a surrogate, a prior distribution and a posterior distribution. Depending on the frameworks used to obtain uncertainty, the prior or the posterior may not exist under certain circumstances. However, every process must have a surrogate. Overall, process acts as a control over surrogate and the distributions of its parameter, and provides one-to-one match between them. This is very important for some problems, where different surrogates may share the same parameter. Details will be discussed later {\color{blue}{refer the section here}}.

{\color{blue} {The fifth paragraph describes how we categorize UQ frameworks, and how frameworks in different types connect to components in different types.}}

As shown in Fig 3, the library currently supports three frameworks for UQ, referred as \textit{Samplable} one, \textit{Trainable} one and \textit{Variational} one, each one of which has its own unique composition of processes, likelihoods and inference methods. \textit{Samplable} framework represents the ones where Bayesian model is considered, process's prior is present and posterior is not, and Markov Chain Monte Carlo (MCMC) inference methods are used. In this case, direct sampling is performed on the un-normalized posterior distribution to obtain posterior samples. The word \textit{Samplable} indicates that parameters are sampled and not trained. \textit{Trainable} framework represents the ones where standard NN model is considered, process's posterior is present and prior is not, and standard NN training is performed. The word \textit{Trainable} indicates that posterior samples are obtained through training. \textit{Variational} framework represents the ones where Bayesian model, particularly variational model, is considered, both process's prior and proposed parameterized posterior are present, and the real posterior is approximated by optimizing some distance, e.g. KL-divergence, between the true posterior and the proposed one. The word \textit{Variational} indicates that it is a variational inference framework, and posterior samples are obtained by sampling the proposed distribution, after the optimization.

\subsection{Usage}\label{usage}

As discussed in Section \ref{sec:overview}, the most crucial functionality of the library is to obtain posterior samples. To that end, in the design phase, a model is constructed such that it includes processes representing the solution $u$ and potentially $f$ and/or $\lambda$; as well as likelihood/loss functions representing the data distribution. The general workflow of the library is presented in Procedure \ref{alg:uq4sciml}. We will discuss the built-in primitive components of the library, as well as their customizability in the next section.

\begin{algorithm}[htbp]
\caption{Usage of UQ4SciML for solving differential equations.}
\label{alg:uq4sciml}
\begin{enumerate}
\item[Step 1] Specify the surrogate for the solution to a differential equation using the \textbf{\texttt{process}} module.
\item[Step 2] Specify the differential equation using the automatic differentiation.
\item[Step 3] Construct the likelihoods or loss functions based on the equations, boundary/initial conditions, and or given data, using the \textbf{\texttt{losses}} module.
\item[Step 4] Combine the process and likelihoods/loss functions to construct a \textbf{\texttt{model}}.
\item[Step 5] Specify the inference method using the \textbf{\texttt{inference}} module.
\item[Step 6] Call \textbf{\texttt{model.compile}} for initialization of the hyperparameters, such as initial values for weights/biased in HMC, optimizer and learning rate, etc.
\item[Step 7] Call \textbf{\texttt{model.run}} to train the network to obtain the optimal hyperparameters. 
\item[Step 8] Feed the hyperparameters obtained at Step 7 to the surrogate from Step 1 to get the predicted functional samples.
\end{enumerate}
\end{algorithm}

\begin{figure}[!ht]
	\centering
	\includegraphics[width=.9\linewidth]{./figs/design1.png}
	\caption{Library design overview.
	In the design phase, a model is constructed that includes processes representing a proposed solution family and likelihood or loss functions representing the data distribution.
	Processes include surrogates, which can be construed as assumed functional forms, and priors distributions or variables for the parameters of the surrogates, depending on the type of method used.
    Likelihoods or loss functions are constructed using the data and the underlying neural ODE/PDE.
    To select the solution function samples that best explain the data, a posterior inference method is combined with the model.
    Finally, the obtained function samples can be calibrated using additional data. 
    In the revision phase, metrics are used for evaluating the performance and re-designing the solution procedure.
	}
	\label{fig:lib:overview}
\end{figure}

\subsection{Components and their customizability}\label{customizability}
As discussed in previous sections and shown in  Fig. \ref{fig:lib:overview}, there are five main components in the library: surrogates, variables, processes, likelihoods and inference methods. Also notice that the library supports three distinct frameworks for UQ in SciML, and compatibility issue needs to be taken care of before using the library.
For example, \textit{Samplable} variables can not work as posterior for \textit{Variational} framework, because they do not have proposed, parameterized distributions, which is necessary for \textit{Variational} framework. In this section, we will discuss those components one by one, show their compatibility and customizability.

\subsubsection{Surrogates} As discussed above, surrogates are parameterized by $\theta$ and when combined with $\theta$'s probability distribution result to stochastic processes; i.e. a proposed family of solutions. The library current supports four common built-in surrogates, \textbf{\texttt{surrogates.identity}}, \textbf{\texttt{fnn}}, \textbf{\texttt{generator}} and \textbf{\texttt{deeponet}}. The \textbf{\texttt{identity}} represents a identity function, which is commonly used when a constant is unknown; \textbf{\texttt{fnn}} represents a fully-connected neural network; \textbf{\texttt{generator}} represents the generator of a pre-trained PI-GAN, which is used as an informative surrogate trained on historical data \cite{meng2022learning}; \textbf{\texttt{deeponet}} represents a DeepONet with only one branch net and one trunk net. It is worth noting that surrogates have the highest compatibility, and in most cases, they are shared across all frameworks. This high compatibility of surrogates comes from how we decompose the whole problem: the uniqueness of framework only shows on estimating surrogates' parameters, instead of themselves.

Users may want to deploy their own surrogates. For example, this happens when more informative surrogates are available, or a different type of neural networks are needed for different problems. One example is shown in \ref{sec:sine}, where the same problem is tackled using different surrogates on the same data, each of which represent a different level of prior knowledge. A new surrogate can be defined as shown in Procedure \ref{alg:surrogates}. Notice that a surrogate instance works as a Python callable, and hence its ``\_\_call\_\_'' method has to be overwritten.


\begin{algorithm}[htbp]
\caption{Customization of surrogates.}
\label{alg:surrogates}
\begin{lstlisting}
from surrogates import Surrogate

class MySurrogate(Surrogate):
    def __call__(self, inputs, var_list):
        """Returns the outputs of the surrogate(s) to the input `inputs`, defined by samples stored in `var_list`."""
\end{lstlisting}
\end{algorithm}

\subsubsection{Variables} The library refers parameters of the surrogates, $\theta$, as variables. Different surrogate has different variables. For example, a \textbf{\texttt{fnn}}'s variables are its weights and biases, while a \textbf{\texttt{generator}}'s variable is the input to the generator. Consistent with the UQ frameworks, variables are also defined in three different types, \textit{Samplable}, \textit{Trainable} and \textit{Variational}. They share some common features but also differ from each other. For example, \textit{Samplable} variables uniquely have initial values, which are used to initialize Markov chains in MCMC methods; both \textit{Samplable} variables and \textit{Variational} variables have methods ``log\_prob'' to compute log probability density of groups of samples on their own distributions.

In the library, the built-in primitive distribution for \textit{Samplable} and \textit{Variational} variables is Gaussian distribution, which is the most common distribution used as the prior and proposed posterior distributions of neural networks' weights and biases. \textit{Trainable} framework is not Bayesian in nature, but regularization can be imposed on \textit{Trainable} variablesm as the counterpart of prior distribution in Bayesian framework. For example, Normal prior distribution for a \textit{Samplable} variable in Bayesian framework, is equivalent to $L_2$ regularization for a \textit{Trainable} variable in MAP (maximum a posteriori).

Most of times, we customize variables for the following two reasons: we want to change the prior/regularization in \textit{Samplable}/\textit{Trainable} frameworks; we want to change the way of parameterizing the posterior distribution in \textit{Variational} framework. As shown in \cite{psaros2022uncertainty}, different prior induces significantly different uncertainties. As for the latter reason, one example is shown in \ref{sec:vi}, where the same problem is solved using the same surrogate but different parameterized distributions. A new variable can be defined as shown in Procedure \ref{alg:variables}. 

\begin{algorithm}[htbp]
\caption{Customization of variables.}
\label{alg:variables}
\begin{lstlisting}
from variables import _Trainable, _Samplable, _Variational
class MyTrainable(_Trainable):
    @property
    def trainable_variables(self):
        """Returns the variable's trainable variables."""
        
    @property
    def losses(self):
        """Returns the variable's regularization loss."""
        
class MySamplable(_Samplable):
    @property
    def initial_values(self):
        """Returns the variable's initial values."""
        
    def log_prob(self, samples):
        """Returns the log probability density of `samples`."""
        
class MyVariational(_Variational):
    @property
    def trainable(self):
        """Returns whether the variable is trainable (optimizable as a parameterized distribution)."""
    def log_prob(self, samples):
        """Returns the log probability density of `samples`."""
    
    def sample(self, sample_shape=[]):
        """Returns `sample_shape` realizations of the variable."""

\end{lstlisting}
\end{algorithm}

\subsubsection{Processes}

In the library, processes are used to identify frameworks, integrate surrogates and variables, as well as assign and receive samples. 

As introduced before, a process consists of three main components, a surrogate, a prior and a posterior. For clarification, here posterior does not mean the posterior distribution of $\theta$ given data $\cD$. Instead, it means the proposed parameterized distribution, used to approximate the real posterior by optimizing some metrics, e.g. ELBO.

\subsubsection{Likelihoods}

\subsubsection{Inference methods}

==> IN_sciml.tex <==
In this section, we first briefly describe various SciML problem scenarios and the recently developed deep learning methods for solving them.  Subsequently, we review the related UQ methods as well as the approaches for model performance evaluation and for post-training calibration.  We also provide 
a table of glossary for the frequently used terms of ML/SciML in Appendix \ref{sec:glossary}. 
The interested reader is directed to \cite{psaros2022uncertainty} for more detailed information regarding SciML problem scenarios and UQ methods.

\subsection{Scientific machine learning}
\label{sec:uqINsciml:sciml}

Consider a nonlinear ordinary/partial differential equation (ODE/PDE) describing the dynamics of a physical system as follows:
\begin{subequations}\label{eq:intro:piml:pinn:pde}
	\begin{align}
		\pazocal{F}_{\lambda, \xi}[u(x; \xi)] &= f(x; \xi) \text{, } x \in  \Omega\text{, } \xi \in \Xi, 
		\label{eq:intro:piml:pinn:pde:a}\\
		\pazocal{B}_{\lambda, \xi}[u(x; \xi)] & = b(x; \xi) \text{, } x \in \Gamma, 
		\label{eq:intro:piml:pinn:pde:b}
	\end{align}
\end{subequations}
where $x$ is the $D_x$-dimensional space-time coordinate, $\Omega$ is a bounded domain with boundary $\Gamma$, $\xi$ is a random event in a probability space $\Xi$, while $f(x; \xi)$ and $u(x; \xi)$ represent the $D_u$-dimensional source term and sought solution evaluated at $(x, \xi)$, respectively. 
Further, $\pazocal{F}_{\lambda, \xi}$ is a general differential operator; $\pazocal{B}_{\lambda, \xi}$ is a boundary/initial condition operator acting on the domain boundary $\Gamma$; and $b$ is a boundary/initial condition term.
Furthermore, $\lambda(x; \xi)$, with $x \in \Omega_{\lambda} \subset \Omega$, denotes the problem parameters.
We refer to problems where the operators $\pazocal{F}_{\lambda, \xi}$ and $\pazocal{B}_{\lambda, \xi}$ are known, i.e., the differential operators that define them are specified, as \textit{neural ODEs/PDEs}, because we use neural networks (NNs) throughout the present work to solve them.
We refer to problems involving unknown operators $\pazocal{F}_{\lambda, \xi}$ and $\pazocal{B}_{\lambda, \xi}$ as \textit{neural operators}, because we use NNs to learn them. 

For neural ODEs/PDEs, $\pazocal{F}_{\lambda, \xi}$, $\pazocal{B}_{\lambda, \xi}$ are deterministic and known, while $\lambda(x), u(x)$ are partially unknown. 
Given noisy data of $u$ and $\lambda$ sampled at random finite locations in $\Omega$ and $\Omega_{\lambda}$, respectively, as well as noisy data of $f$ and $b$, the objective of this problem is to obtain the solution $u(x)$ at every $x \in \Omega$ and the problem parameters $\lambda(x)$ at every $x \in \Omega_{\lambda}$.
The dataset in this case is expressed as $\cD = \{\cD_f, \cD_b, \cD_u, \cD_{\lambda}\}$, where $\cD_u = \{x_i, u_i\}_{i=1}^{N_u}$, $\cD_{\lambda} = \{x_i, \lambda_i\}_{i=1}^{N_{\lambda}}$, $u_i = u(x_i)$, $\lambda_i = \lambda(x_i)$, and $\cD_f, \cD_b$ are given as above.
The PINN method, developed in \cite{raissi2019physicsinformed}, addresses the forward deterministic PDE problem by constructing a NN approximator, parametrized by $\theta$, for modeling the solution $u(x)$.
The approximator $u_{\theta}(x)$ is substituted into Eq.~\eqref{eq:intro:piml:pinn:pde} via automatic differentiation for producing $f_{\theta} = \pazocal{F}_{\lambda}[u_{\theta}]$ and $b_{\theta} = \pazocal{B}_{\lambda}[u_{\theta}]$.
For solving the mixed deterministic PDE problem, an additional NN can be constructed for modeling $\lambda(x)$.
Finally, the optimization problem for obtaining $\theta$ in the mixed problem scenario with the dataset $\cD = \{\cD_f, \cD_b, \cD_u, \cD_{\lambda}\}$ is cast as
\begin{multline}\label{eq:intro:piml:pinn:loss:1}
	\hat{\theta} = \underset{\theta}{\mathrm{argmin}}~\pazocal{L}(\theta) \text{, where } 
	\pazocal{L}(\theta) = \frac{w_f}{N_f}\sum_{i=1}^{N_f}
		||f_{\theta}(x_i) - f_i||_2^2 \\ +
	 \frac{w_b}{N_b}\sum_{i=1}^{N_b}
		||b_{\theta}(x_i)-b_i||_2^2
	+  \frac{w_u}{N_u}\sum_{i=1}^{N_u}
		||u_{\theta}(x_i) - u_i||_2^2
	+ \frac{w_{\lambda}}{N_{\lambda}}\sum_{i=1}^{N_{\lambda}}
		||\lambda_{\theta}(x_i) - \lambda_i||_2^2.
\end{multline}
In this equation, $\{w_f, w_b, w_u, w_{\lambda}\}$ are objective function weights for balancing the various terms in Eq.~\eqref{eq:intro:piml:pinn:loss:1}.
Following determination of $\hat{\theta}$, $u_{\hat{\theta}}$ and $\lambda_{\hat{\theta}}$ can be evaluated at any $x$ in $\Omega$, $\Omega_{\lambda}$, respectively.

For neural operators, $\pazocal{F}_{\lambda, \xi}$, $\pazocal{B}_{\lambda, \xi}$ are stochastic and unknown, while $\lambda(x; \xi), u(x; \xi)$ are partially unknown. {\color{blue}{For operator learning, it should state that stochasticity of $\lambda(x, \xi)$ and $u(x, \xi)$ induces the whole stochasiticity of $\pazocal{F}_{\lambda, \xi}$ and $\pazocal{B}_{\lambda, \xi}$. In other word, once $\lambda$ and $u$ are certain, the operators should also be certain.}}
The available data consists of paired realizations of $f, b, u$, and $\lambda$, each one associated with a different $\xi \in \Xi$.
The realizations are considered noisy in general for $u$, and clean for $f, b$, and $\lambda$.
Further, the objective of this problem is to learn the operator mapping defined by Eq.~\eqref{eq:intro:piml:pinn:pde}.
We refer to this procedure as \textit{pre-training} and the required dataset is the same as in the mixed stochastic problem, except with clean data for $f, b$, and $\lambda$.
For employing the learned operator during \textit{inference} for an unseen $\xi' \in \Xi$, we are given noisy and limited data of $f, b, u$, and $\lambda$, and the objective is to obtain $f, b, u$, and $\lambda$ at every $x$ in the corresponding domains.  
The inference dataset in this case is expressed as $\cD' = \{\cD_f', \cD_b', \cD_u', \cD_{\lambda}'\}$, where $\cD_f' = \{x_i, f_i\}_{i=1}^{N_f'}$, $\cD_b' = \{x_i, b_i\}_{i=1}^{N_b'}$, $\cD_u' = \{x_i, u_i\}_{i=1}^{N_u'}$, and $\cD_{\lambda}' = \{x_i, \lambda_i\}_{i=1}^{N_{\lambda}'}$.
Finally, note that a special case of inference data is where $f, b$ and $\lambda$ data are available at the complete set of locations used in pre-training, and the only sought outcome is the solution $u$.
The DeepONet method, developed in \cite{lu2021learning}, addresses the special case of the operator learning problem by constructing a NN approximator, parametrized by $\theta$, for modeling the solution $u(x; \xi)$.
In the following and without loss of generality, we consider $f$ and $b$ in Eq.~\eqref{eq:intro:piml:pinn:pde} as known. 
Further, each value of $\xi \in \Xi$ in Eq.~\eqref{eq:intro:piml:pinn:pde} corresponds to a different $\lambda(x; \xi)$ function, and thus a different solution $u(x; \xi)$. 
The NN $u_{\theta}(x; \xi)$ takes as input the $\lambda_j^{(i)}$ values from the sub-dataset $\Lambda_i = \{x_j^{(i)}, \lambda_j^{(i)}\}_{j=1}^{N_{\lambda}}$.
The locations $\{x_j^{(i)}\}_{j=1}^{N_{\lambda}}$ are considered the same for all $i$ values, without loss of generality.
The DeepONet architecture consists of two sub-networks, one for the input $x$, called trunk net, and one for the input $\lambda$, called branch net.
Considering a one-dimensional output $u_{\theta}(x; \xi)$, i.e., $D_u=1$, each of the two networks produces a $w$-dimensional output.
The two outputs are merged by computing their inner product for producing the final prediction $u_{\theta}(x; \xi)$.
For learning the operator mapping from $\lambda$ to $u$ with the DeepONet method, the minimization problem with the MSE loss
\begin{equation}\label{eq:intro:piml:don:min}
	\hat{\theta} =  \underset{\theta}{\mathrm{argmin}}~\pazocal{L}(\theta) \text{, where } 
	\pazocal{L}(\theta) = \frac{1}{NN_u}\sum_{i=1}^{N}\sum_{j=1}^{N_u}
	||u_{\theta}(x_j^{(i)}; \xi_i) - u_j^{(i)}||_2^2    
\end{equation}	
is solved. 
% We refer to this procedure as pre-training or just training, depending on whether the inference data is limited and noisy, and requires further processing, or clean and can be directly used for inference.
During inference for a new value $\xi' \in \Xi$, the vanilla DeepONet considers a clean dataset $\cD_{\lambda}' = \{x_i, \lambda_i\}_{i=1}^{N_{\lambda}'}$. 
The corresponding solution $u(x; \xi')$ can be obtained for each required $x \in \Omega$ by performing a forward DeepONet pass.


% If the inference dataset is not clean, a Bayesian NN (BNN) or a Generative Adversarial Network (GAN) functional prior (GAN-FP) is attached to a pre-trained DeepONet. 
% Subsequently, posterior inference is performed for the BNN parameters or the GAN-FP input, for each new value $\xi' \in \Xi$.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Uncertainty quantification}\label{sec:uqINsciml:uq}

\begin{figure}[h]
	\centering
	\includegraphics[width=.9\linewidth]{./figs/functional_prior.png}
	\caption{Surrogates employed for learning neural ODEs/PDEs and operators.
	For neural ODEs/PDEs, the solution $u$ is modeled with a surrogate parametrized by $\theta$. 
The surrogate $\cM$ can be a standard NN or a pre-trained GAN functional prior (GAN-FP).
These models are referred to as U-PINN and PI-GAN-FP, respectively, in \cite{psaros2022uncertainty}.
In both cases different $\theta$ values correspond to different functions $u_{\theta}$. 
For the special case of learning neural operators described in Section~\ref{sec:uqINsciml:sciml}, the solution $u$ is modeled with a DeepONet surrogate parametrized by $\theta$ while posterior inference is performed as above. 
This model is referred to as U-DeepONet in \cite{psaros2022uncertainty}.
For the more general case in which the inference input data are noisy, the DeepONet is pre-trained with fixed parameters, and the input $f$ is modeled with a 
Bayesian NN (BNN) or a GAN-FP, denoted by $\cM$.
These models are referred to as PA-BNN-FP and PA-GAN-FP, respectively, in \cite{psaros2022uncertainty}.}
	\label{fig:neurals}
\end{figure}

% {\color{blue}{Use different colors to encode different components in FIG. \ref{fig:neurals}, e.g. one color for the inputs, one color for the parameters, one color for outputs, such that FIG. \ref{fig:neurals}} matches the library.}

As opposed to the point estimates obtained via the optimization problems of Eqs.~\eqref{eq:intro:piml:pinn:loss:1} and \eqref{eq:intro:piml:don:min}, the goal of UQ is to estimate the predictive distribution
\begin{align}\label{eq:pred_dist}
    p(u|x,\cD) = \int p(u|x, \theta) p(\theta | \cD) d\theta,
\end{align}
which is often referred to as Bayesian model average (BMA).
In Eq.~\eqref{eq:pred_dist}, $p(\theta|\cD)$ denotes the \textit{posterior density}, which can be obtained using Bayes' rule via
\begin{equation}\label{eq:uqt:pre:bma:post}
	p(\theta|\cD) =\frac{p(\cD|\theta)p(\theta)}{p(\cD)}.
\end{equation}
In Eq.~\eqref{eq:uqt:pre:bma:post}, $p(\cD|\theta)$ is the likelihood of the data, i.e., $p(\cD|\theta) = \prod_{i=1}^{N}p(u_i|x_i, \theta)$ for independent and identically distributed (i.i.d.) data; $p(\theta)$ is the prior probability of the parameters $\theta$; and $p(\cD)$ is called \textit{marginal likelihood} or \textit{evidence}, because it represents the probability that out of all possible modeled datasets, it ``happens'' that we observe $\cD$.
The evidence is given as
\begin{equation}\label{eq:uqt:pre:bma:marglike}
	p(\cD) =\int p(\cD|\theta)p(\theta) d\theta. 
\end{equation}
The uncertainty of the NN parameters $\theta$ is typically referred to as \textit{epistemic uncertainty}. Generally, inferring $\theta$ given a dataset, i.e., computing the posterior exactly via Eq.~\eqref{eq:uqt:pre:bma:post} is computationally and analytically intractable. 
This is addressed by approximate posterior inference, which approximates the posterior by another distribution and/or obtains representative samples from the posterior. 

The Bayesian and the deterministic frameworks are the two main families of UQ methods for SciML, as reviewed by Psaros et al. \cite{psaros2022uncertainty}. 
The former employs either a sampling method or a variational inference (VI) method to obtain samples from the posterior distribution, whereas the latter can be interpreted as an extension of standard, i.e., deterministic, training of NNs. 
Various UQ methods have been proposed within each of the two frameworks and the rest of this section provides a short overview.
In the following, we adopt the unified framework of Fig. \ref{fig:neurals}, proposed in \cite{psaros2022uncertainty}, to include various UQ models in SciML.

For neural ODEs/PDEs, the solution $u$ is modeled with a \textit{surrogate} parametrized by $\theta$ and denoted by $\cM$ in Fig.~\ref{fig:neurals}.  
In \cite{psaros2022uncertainty}, these models are referred to as U-PINN, and PI-GAN-FP, respectively. 
In all cases, different $\theta$ values correspond to different functions $u_{\theta}$. 
We refer to the surrogate combined with a probability distribution $p(\theta)$ for $\theta$ as a \textit{process}. 
As mentioned earlier in the paper, posterior inference obtains representative $\theta$ samples that explain the data $\cD$, based on the process definition.
Also, the problem parameters $\lambda$ can either be unknown constants or unknown fields depending on the problem setup.  
In such cases, we can use surrogates for $\lambda$, parametrized by $\theta_{\lambda}$. 
Accordingly, posterior inference is performed for both $\theta$ and $\theta_{\lambda}$ simultaneously.

For the special case of learning neural operators described in Section~\ref{sec:uqINsciml:sciml}, the solution $u$ is modeled with a DeepONet surrogate parametrized by $\theta$ and posterior inference is performed as above. 
This model is referred to as U-DeepONet in \cite{psaros2022uncertainty}.
However, for the more general case in which the inference input data are noisy, the DeepONet is pre-trained with fixed parameters, and the input $f$ is modeled with a BNN or a GAN-FP, denoted by $\cM$ in Fig.~\ref{fig:neurals}.
These models are referred to as PA-BNN-FP and PA-GAN-FP, respectively, in \cite{psaros2022uncertainty}. 
Posterior inference is performed as above for the BNN parameters $\theta$ or the GAN input $\theta$. 

% In passing, note that the ensemble posterior inference methods, summarized in Table~\ref{tab:uqt:over}, do not require a prior $p(\theta)$ and thus, we only need to define the surrogate component.

% \subsubsection{Likelihoods}\label{sec:likelihoods}

% Given a set of paired noisy observations $\cD = \{x_i,u_i\}_{i=1}^{N}$, our goal is to construct a distribution $p(u|x, \cD)$ for predicting the value of $u$ at any new location $x$. 
% For each $x$, it is commonly assumed that $u(x)$ produced by the data-generating process contains both a deterministic part $u_c(x)$ as well as some additive noise $\epsilon_u$, i.e., $u(x) = u_c(x) + \epsilon_u$.
% This noise is typically called data or aleatoric uncertainty. 
% For modeling this process, we assume a \textit{likelihood function} denoted by $p(u|x, \theta)$, with parameters $\theta=[\theta_1,\dots,\theta_K]^T$ to be inferred from the available data.
% Further, for defining $p(u|x, \theta)$ we construct a model $u_{\theta}(x)$ that captures the deterministic part of $u(x)$ at some location $x$ and assume a model for the noise.
% For example, the factorized Gaussian likelihood function, given as
% \begin{equation}\label{eq:uqt:pre:bma:Glike}
% 	p(u|x, \theta) = \cN(u|u_{\theta}(x), diag(\Sigma_{u}^2)) = \prod_{d = 1}^{D_u}\frac{1}{\sqrt{2\pi \sigma_{u}^2}}\exp(-\frac{(u_d-u_{\theta}(x)_d)^2}{2\sigma_{u}^2}), 
% \end{equation}
% with the subscript $d$ denoting each of the $D_u$ dimensions of $u$, is often used for multi-dimensional function approximation problems.
% In Eq.~\eqref{eq:uqt:pre:bma:Glike}, the output vector $u_{\theta}(x)$ is the mean of the Gaussian distribution assumed for $u$ at location $x$, $diag(\Sigma_{u}^2)$ is a diagonal covariance matrix with $\Sigma_{u}^2 = [\sigma_{u}^2,\dots,\sigma_{u}^2]$ in the diagonal, and $\sigma_{u}^2$ may either be known or assumed, or inferred from data.

% For neural ODEs/PDEs, the observations in the dataset $\cD = \{\cD_f, \cD_b, \cD_u, \cD_{\lambda}\}$ are typically obtained with a data acquisition device and are noisy. 
% In this regard, we employ four likelihood functions for approximating the $f, b, u$ and $\lambda$ distributions, denoted as $p(f|x, \theta), p(b|x, \theta), p(u|x, \theta)$, and $p(\lambda|x, \theta)$, respectively.
% The total likelihood of the dataset $\cD$ becomes
% \begin{equation}\label{eq:uqt:pre:pinn:like}
% 	p(\cD|\theta) = p(\cD_f|\theta)p(\cD_b|\theta)p(\cD_{u}|\theta)p(\cD_{\lambda}|\theta),
% \end{equation}
% where 
% \begin{equation}
% \begin{aligned}\label{eq:uqt:pre:pinn:likes}
% 	p(\cD_f|\theta) & = \prod_{i=1}^{N_f}p(f_i|x_i, \theta) \text{; } & p(\cD_b|\theta) & = \prod_{i=1}^{N_b}p(b_i|x_i, \theta);\\
% 	p(\cD_u|\theta) & = \prod_{i=1}^{N_u}p(u_i|x_i, \theta) \text{; } & p(\cD_{\lambda}|\theta) & = \prod_{i=1}^{N_{\lambda}}p(\lambda_i|x_i, \theta).
% \end{aligned}
% \end{equation}

% For neural operators, we assume that $f$ and $b$ in Eq.~\eqref{eq:intro:piml:pinn:pde} are known and the dataset $\cD_{\lambda}$ consists of clean data.
% Nevertheless, $\cD_u$ consists of noisy data in general.
% In this regard, a likelihood function is employed for the $u$ data, denoted by $p(u|x, \xi, \theta)$, and the total likelihood is given as
% \begin{equation}\label{eq:uqt:pre:don:like}
%     p(\cD|\theta) =\prod_{i=1}^{N}\prod_{j=1}^{N_u}p(u_j^{(i)}|x_j^{(i)}, \xi_i, \theta). 
% \end{equation}

% \subsubsection{Posterior inference}\label{sec:inference}

% Performing UQ for neural ODEs/PDEs and operators involves combining the constructed model with a posterior inference method. 
% In this section, we provide a summary of the considered inferences for producing surrogate parameter $\theta$ samples and subsequently, the sought function samples.

% Obtaining the posterior distribution of $\theta$ is computationally and analytically intractable. 
% To address this issue, approximate inference aims to approximate the posterior by another distribution and/or obtaining  NN parameter posterior samples $\{\hat{\theta}_j\}_{j=1}^M$ from the posterior.
% In Table~\ref{tab:uqt:over} we provide an overview of the most commonly used methods for obtaining $\{\hat{\theta}_j\}_{j=1}^M$; see Fig.~\ref{tab:uqt:over} and \cite{psaros2022uncertainty} for more details.
% We refer to the HMC, LD, MFVI, and LA methods as \textit{Bayesian}, because they are related with the Bayesian paradigm of obtaining posterior samples, and to the MCD, DEns, SEns, and SWAG methods as \textit{deterministic}, because they can be interpreted as extensions of standard, i.e, deterministic, training of NNs.

% In the package, the default option is to combine the methods with a Bayesian neural network, as a surrogate.
% Alternatively, a GAN functional prior can be used.

%\textcolor{blue}{
%UQ4SciML supports three different types of posterior estimation methods, i.e., sampling-based method, vi-based method, and . Specifically, the sampling- and vi-based posterior estimations are for \textit{Bayesian} methods, and the .  MCMC-based methods utilize Markov chain Monte Carlo to sample directly against, probably un-normalized, posterior distribution. We describe MCMC-based methods as sampling methods. Ensemble-based methods execute standard training of NNs, throughout which samples are collected to group an ensemble. We describe such methods as sampling-through-optimization ones. Finally, VI-based methods are closely related with variational inferences, where posterior is approximated by optimizing some distance, e.g. KL-divergence, between the real one and a parameterized one. After the optimization completes, samples are obtained by sampling against the trained parameterized distribution, and hence we describe such methods as optimizing-and-sampling ones. Types of inference methods should be consistent with the type of model, e.g. an MCMC-based method can not work with a variational inference model, even though they both belong to the family of Bayesian inference.
%}

% \subsubsection{From parameter to function samples}\label{sec:fsamples}

Following approximate posterior inference, the posterior samples for $\theta$ are used for obtaining the statistics of the function samples.
In this regard, the value of $u$ at a location $x$ given the data $\cD$ is a random variable denoted by $(u|x, \cD)$.
The mean of $(u|x, \cD)$ is denoted by $\hat{u}(x) = \mathbb{E}[u|x, \cD]$ and approximated by $\bar{\mu}(x)$ as
\begin{equation}\label{eq:uqt:pre:mcestmc:mean}
	\hat{u}(x) \approx \bar{\mu}(x) = \frac{1}{M}\sum_{j=1}^Mu_{\hat{\theta}_j}(x),
\end{equation}
where $\{u_{\hat{\theta}_j}(x)\}_{j=1}^M$ is the set of NN predictions corresponding to the samples $\{\hat{\theta}_j\}_{j=1}^M$.
Further, the diagonal part of the covariance matrix of $(u|x, \cD)$ is given by
\begin{equation}\label{eq:uqt:pre:mcestmc:totvar}
	Var(u|x, \cD) \approx \bar{\sigma}^2(x) =  \underbrace{\Sigma_{u}^2}_{\bar{\sigma}_a^2(x)}  + \underbrace{\frac{1}{M}\sum_{j=1}^M(u_{\hat{\theta}_j}(x)-\bar{\mu}(x))^2}_{\bar{\sigma}_e^2(x)}. 
\end{equation} 
In this equation, $\bar{\sigma}^2(x)$ represents the approximate total uncertainty of $(u|x, \cD)$, while $\bar{\sigma}_a^2(x)$ and $\bar{\sigma}_e^2(x)$ denote the aleatoric and the epistemic parts of the total uncertainty, respectively.
In practice, a Gaussian (or, e.g., a Student-t) distribution is commonly fitted to the posterior samples.
For example, we denote as $\pazocal{N}(\bar{\mu}(x), \bar{\sigma}^2(x))$ the Gaussian approximation to the samples $\{u_{\hat{\theta}_j}(x)\}_{j=1}^M$ at an arbitrary location $x$, where $\bar{\mu}(x)$ and $\bar{\sigma}^2(x)$ are obtained via Eqs.~\eqref{eq:uqt:pre:mcestmc:mean} and \eqref{eq:uqt:pre:mcestmc:totvar}, respectively.

\subsection{Performance evaluation and post-training calibration}\label{sec:calibration}


\begin{table}[h]
	\centering
	\footnotesize
	\begin{tabular}{clc}
		\toprule
		\multicolumn{3}{c}{\textbf{Post-training calibration methods}}\\
		\midrule
		Reference & Short description & Name in library
		\\
		\midrule
		\multirow{2}{*}{\cite{levi2019evaluating}}  &  Re-weighting optimally all predicted variances. & \multirow{2}{*}{\textbf{\texttt{calibration.var}}} \\
		 & Modifies only the variance of the predictions. & \\
		\arrayrulecolor{black!30}\midrule
		\multirow{3}{*}{\cite{kuleshov2018accurate}} &  Approximates misscalibration function & \textbf{\texttt{calibration.cdf}}
		\\ & and applies it to all predictive distributions. & (not currently
         \\ & Modifies both the mean and the variance of all predictions. & implemented)\\
		\arrayrulecolor{black!30}\midrule
		\multirow{3}{*}{\cite{zelikman2020crude}} & An empirical distribution is fitted to the scaled residuals & \textbf{\texttt{calibration.crude}}
		\\ & that correspond to the calibration dataset.& (not currently
		\\& Modifies both the mean and the variance of all predictions.& implemented) \\ 
		\arrayrulecolor{black}
		\bottomrule
	\end{tabular}
	\caption{Overview of the post-training calibration methods considered in this paper. 
	These methods can be used for improving statistical consistency; i.e., how closely the predictive model matches the data-generating distribution.
    To that end, an additional dataset $\cD_r = \{x_i, u_i\}_{i=1}^{N_r}$ is required after training.
    This can be a left-out calibration dataset, similar to validation and test sets.
	}
	\label{tab:calibration}
\end{table}

Performance evaluation is necessary for model
selection, e.g., prior/architecture optimization, comparison between UQ methods, and overall quality evaluation of the UQ design procedure.
As reviewed in \cite{psaros2022uncertainty}, performance evaluation metrics include the relative $\ell_2$ error for evaluating accuracy, the mean predictive likelihood for evaluating predictive capacity, and the root mean squared calibration error for evaluating statistical consistency; i.e., how closely the predictive model matches the data-generating distribution.


Further, for improving statistical consistency, we provide in Table~\ref{tab:calibration} three post-training calibration approaches.
To use these approaches an additional dataset $\cD_r = \{x_i, u_i\}_{i=1}^{N_r}$ is required after training.
This can be a left-out calibration dataset, similar to validation and test sets.

==> IN_sciml2.tex <==
In this section, we first briefly describe various SciML problem scenarios and the recently developed deep learning methods for solving them.  Subsequently, we review the related UQ methods as well as the approaches for model performance evaluation and for post-training calibration.  We also provide 
a table of glossary for the frequently used terms of ML/SciML in Appendix \ref{sec:glossary}. 
The interested reader is directed to \cite{psaros2022uncertainty} for more detailed information regarding SciML problem scenarios and UQ methods.

% The interested reader can also direct to \cite{psaros2022uncertainty} for more detailed information. 
% {\color{blue} {In this section, we briefly discuss recent advances in SciML and associated uncertainty quantification techniques. We present, in a very general way, an overview of problems are solvable using machine learning, particularly neural networks, and methods used to address those problems, which includes PINN, PI-GAN, PI-GAN-FP and DeepONet. Next, we discuss common UQ frameworks developed recently for SciML, which are closely related to the methods we mentioned above. Some methods may have multiple UQ versions, representing multiple frameworks to obtain uncertainty. We briefly discuss how we formulate the UQ problems, how we solve them in various ways, and how different framework differs from each other.}}

% {\color{blue}{Subsection 1: NN for SciML, PINN, PI-GAN, DeepONet.}}
% {\color{blue}{Subsection 2: Plurality of UQ frameworks. For PINN, we have B-PINN, U-PINN. U-PINN represents a deterministic framework, which further induces \textit{Trainable} framework for UQ4PINN in the next section. B-PINN represents a Bayesian framework for UQ, which splits into two subframeworks, the one where sampling methods are directly used and the one where a proposed distribution is used to approximate the target distribution, which induces \textit{Samplable} and \textit{Variational} frameworks in the next sections. For PI-GAN, we have PI-GAN-FP, which may solved using all three frameworks. Finally, for DeepONet, we have U-DeepONet, which may only be used using one framework. }}

% {\color{red} {ZZ's comment: besides problem formulation and related works in SciML, with or without UQ, I want to highlight two things in this section. One, every regular method, PINN, PI-GAN, DeepONet has its extended UQ version. Two, each UQ version can be tackled in one-to-three ways. The second highlight matches the library design in section 3 perfectly.}}



\subsection{Scientific machine learning}
\label{sec:uqINsciml:sciml}

Consider a nonlinear ordinary/partial differential equation (ODE/PDE) describing the dynamics of a physical system as follows:
\begin{subequations}\label{eq:intro:piml:pinn:pde}
	\begin{align}
		\pazocal{F}[x;u(x);\lambda(x)] &= f(x) \text{, } x \in  \Omega, 
		\label{eq:intro:piml:pinn:pde:a}\\
		\pazocal{B}[x;u(x);\lambda(x)] & = b(x) \text{, } x \in \Gamma,
		\label{eq:intro:piml:pinn:pde:b}
	\end{align}
\end{subequations}
where $x$ is the $D_x$-dimensional space-time coordinate, $\Omega$ is a subset of $\mathbb{R}^{D_x}$ with boundary $\Gamma$, while $f(x)$ and $u(x)$ represent the $D_u$-dimensional source term and sought solution evaluated at $x$, respectively. 
Further, $\pazocal{F}$ is a general nonlinear operator; $\pazocal{B}$ is a boundary/initial condition operator acting on the domain boundary $\Gamma$; and $b$ is a boundary/initial condition term. Furthermore, $\lambda(x)$ denotes the problem parameters. In this study, we refer to problems in which (1) $\pazocal{F}$ and/or $\pazocal{B}$ are known as \textit{physics-informed learning} problems, and (2) $\pazocal{F}$ and/or $\pazocal{B}$ are unknown or partially known as \textit{physics-agnostic learning} problems. 

%We refer to problems where the operators $\pazocal{F}_{\lambda, \xi}$ and $\pazocal{B}_{\lambda, \xi}$ are known, i.e., the differential operators that define them are specified, as \textit{neural ODEs/PDEs}, because we use neural networks (NNs) throughout the present work to solve them.
%We refer to problems involving unknown operators $\pazocal{F}_{\lambda, \xi}$ and $\pazocal{B}_{\lambda, \xi}$ as \textit{neural operators}, because we use NNs to learn them. 
% {\color{blue}{Physics informed learning: PINN, PI-GAN in SciML, correspond to B-PINN, FP in the UQ section}}


For physics informed learning, the operators $\pazocal{F}$ and $\pazocal{B}$ are known, while $u, \lambda, f, b$ are at least partially known. 
Given noisy data of $u$ and $\lambda$ sampled at random finite locations in $\Omega$ and $\Omega_{\lambda}$, respectively, as well as noisy data of $f$ and $b$, the objective of this problem is to obtain the solution $u(x)$ at every $x \in \Omega$ and the problem parameters $\lambda(x)$ at every $x \in \Omega_{\lambda}$.
The dataset in this case is expressed as $\cD = \{\cD_f, \cD_b, \cD_u, \cD_{\lambda}\}$, where $\cD_u = \{x_i, u_i\}_{i=1}^{N_u}$, $\cD_{\lambda} = \{x_i, \lambda_i\}_{i=1}^{N_{\lambda}}$, $u_i = u(x_i)$, $\lambda_i = \lambda(x_i)$, and $\cD_f, \cD_b$ are given as above.
The PINN method, developed in \cite{raissi2019physicsinformed}, addresses the PDE problem by constructing NN approximators, parameterized by $\theta$, for modeling the solution $u$ and/or parameter $\lambda$. The approximators are substituted into Eq.~\eqref{eq:intro:piml:pinn:pde} via automatic differentiation for producing $f_{\theta} = \pazocal{F}[x; u_{\theta}; \lambda]$ and $b_{\theta} = \pazocal{B}[x; u_{\theta}; \lambda]$.
For solving the mixed and inverse PDE problems, parameterizations of $\lambda$ are also needed.
Finally, the optimization problem for obtaining $\theta$ in the mixed problem scenario with the dataset $\cD = \{\cD_f, \cD_b, \cD_u, \cD_{\lambda}\}$ is cast as
\begin{multline}\label{eq:intro:piml:pinn:loss:1}
	\hat{\theta} = \underset{\theta}{\mathrm{argmin}}~\pazocal{L}(\theta) \text{, where } 
	\pazocal{L}(\theta) = \frac{w_f}{N_f}\sum_{i=1}^{N_f}
		||f_{\theta}(x_i) - f_i||_2^2 \\ +
	 \frac{w_b}{N_b}\sum_{i=1}^{N_b}
		||b_{\theta}(x_i)-b_i||_2^2
	+  \frac{w_u}{N_u}\sum_{i=1}^{N_u}
		||u_{\theta}(x_i) - u_i||_2^2
	+ \frac{w_{\lambda}}{N_{\lambda}}\sum_{i=1}^{N_{\lambda}}
		||\lambda_{\theta}(x_i) - \lambda_i||_2^2.
\end{multline}
In this equation, $\{w_f, w_b, w_u, w_{\lambda}\}$ are objective function weights for balancing the various terms in Eq.~\eqref{eq:intro:piml:pinn:loss:1}.
Following determination of $\hat{\theta}$, $u_{\hat{\theta}}$ and $\lambda_{\hat{\theta}}$ can be evaluated at any $x$ in $\Omega$, $\Omega_{\lambda}$, respectively. The PI-GAN method \cite{yang2020physicsinformed}, although was originally proposed to solve stochastic differential equations and uses an entirely different optimization framework, also belongs to the family of physics-informed learning and can be used to solve PDE problems as well \cite{meng2021learning}.

For physics agnostic learning, $\pazocal{F}$, $\pazocal{B}$ are unknown, while $u, \lambda, f, b$ are partially known. The available data consists of paired realizations of $u, \lambda, f$, and $b$, which are considered noisy in general for $u$, and clean for $f, b$, and $\lambda$. The objective of physics agnostic problems is to learn the underlying physics {\color{red}{the solution operator?}} of Eqs.~\eqref{eq:intro:piml:pinn:pde} from measurements. The DeepONet method, developed in \cite{lu2021learning}, was originally designed for general nonlinear operator learning, addresses this type of problem by constructing an approximator using NNs, $G_\theta$, parameterized by $\theta$, to model the mapping from the input function to the output function. Without loss of generality, we consider both $f$ and $b$ in Eq.~\eqref{eq:intro:piml:pinn:pde} as known and the problem becomes learning the mapping from the parameter $\lambda$ to the solution $u$. The approximator $G_\theta$ takes as input a finite representation of $\lambda(x), x\in \Omega_\lambda$ and outputs a function, $G_\theta(\lambda)(x), x\in \Omega$. 
The DeepONet architecture consists of two sub-networks, one takes the coordinates $x\in\Omega$ as input, called trunk net, and one takes the discretized function $\lambda$ as input, called branch net.
Considering a one-dimensional $u$, i.e., $D_u=1$, each of the two networks produces a $w$-dimensional output.
The two outputs are merged by computing their inner product for producing the final prediction $G_\theta(\lambda)(x), x\in\Omega$.
For learning the mapping from $\lambda$ to $u$ using the vanilla DeepONet \cite{lu2021comprehensive}, the minimization problem with the MSE loss
\begin{equation}\label{eq:intro:piml:don:min}
	\hat{\theta} =  \underset{\theta}{\mathrm{argmin}}~\pazocal{L}(\theta) \text{, where } 
	\pazocal{L}(\theta) = \frac{1}{NM}\sum_{i=1}^{N}\sum_{j=1}^{M}
	||G_{\theta}(\lambda^{(j)})(x_i) - u_i^{(j)}||_2^2    
\end{equation}	
is solved, with the dataset expressed as $\cD' = \{x_i, \lambda^{(j)}, u^{(j)}_i\}_{i,j=1}^{i=N, j=M}$, where $N$ is the number of realizations on $\Omega$ and $M$ is the number of pairs of $\lambda$ and $u$. DeepONets, once trained, could act as PDE-agnostic surrogates with encoded physical knowledge for further learning and inferences \cite{meng2021learning}.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Uncertainty quantification}\label{sec:uqINsciml:uq}

\begin{figure}[h]
	\centering
	\includegraphics[width=.9\linewidth]{./figs/functional_prior.png}
	\caption{Surrogates employed for solution and operator learning.
	For solution learning, the $u$ is modeled with a surrogate parameterized by $\theta$. 
The surrogate $\cM$ can be a standard NN or a pre-trained functional prior (FP).
Different $\theta$ values correspond to different functions $u_{\theta}$. 
For operator learning, the solution $u$ is modeled with a DeepONet surrogate parameterized by $\theta$.
DeepONet, when pre-trained, could be utilized as a fixed surrogate, connecting $f$ and $u$.
}
	\label{fig:neurals}
\end{figure}

% {\color{blue}{Use different colors to encode different components in FIG. \ref{fig:neurals}, e.g. one color for the inputs, one color for the parameters, one color for outputs, such that FIG. \ref{fig:neurals}} matches the library.}

As opposed to the point estimates obtained via the optimization problems of Eqs.~\eqref{eq:intro:piml:pinn:loss:1} and \eqref{eq:intro:piml:don:min}, the goal of UQ is to estimate the predictive distribution
\begin{align}\label{eq:pred_dist}
    p(u|x,\cD) = \int p(u|x, \theta) p(\theta | \cD) d\theta,
\end{align}
which is often referred to as Bayesian model average (BMA).
In Eq.~\eqref{eq:pred_dist}, $p(\theta|\cD)$ denotes the \textit{posterior density}, which can be obtained using Bayes' rule via
\begin{equation}\label{eq:uqt:pre:bma:post}
	p(\theta|\cD) =\frac{p(\cD|\theta)p(\theta)}{p(\cD)}.
\end{equation}
In Eq.~\eqref{eq:uqt:pre:bma:post}, $p(\cD|\theta)$ is the likelihood of the data, i.e., $p(\cD|\theta) = \prod_{i=1}^{N}p(u_i|x_i, \theta)$ for independent and identically distributed (i.i.d.) data; $p(\theta)$ is the prior probability of the parameters $\theta$; and $p(\cD)$ is called \textit{marginal likelihood} or \textit{evidence}, because it represents the probability that we observe $\cD$ out of all possible modeled datasets.
The evidence is given as
\begin{equation}\label{eq:uqt:pre:bma:marglike}
	p(\cD) =\int p(\cD|\theta)p(\theta) d\theta. 
\end{equation}
The uncertainty of parameters $\theta$ is typically referred to as \textit{epistemic uncertainty}. Generally, inferring $\theta$ given $\cD$, i.e., computing the posterior exactly via Eq.~\eqref{eq:uqt:pre:bma:post} is computationally and analytically intractable. 
This is addressed by approximate posterior inference, which approximates the posterior by another distribution and/or obtains representative samples from the posterior. 

The Bayesian and the deterministic frameworks are the two main families of UQ methods for SciML.
The former employs either a sampling method or a variational inference (VI) method to obtain samples from the posterior distribution, whereas the latter can be interpreted as an extension of standard, i.e., deterministic, training of NNs. 
Various UQ methods for SciML have been proposed within each of the two frameworks and the rest of this section provides a short overview.
In the following, we adopt the unified framework of Fig. \ref{fig:neurals}, proposed in \cite{psaros2022uncertainty}, to include various UQ models in SciML.

% {\color{blue}{B-PINN, FP, and DeepONet are the foundation of the library.}}

For physics-informed learning, the solution $u$ and/or the problem parameters $\lambda$ are modeled with a \textit{surrogate} parametrized by $\theta$ and denoted by $\cM$ in Fig. \ref{fig:neurals}. The Bayesian PINNs (B-PINNs) \cite{yang2020bayesian} and the functional prior based on the physics-informed generative adversarial networks (PI-GANs) \cite{meng2021learning,yang2020physicsinformed} are two recently proposed UQ-induced physics-informed learning approaches within the Bayesian framework. The Bayesian neural networks (BNNs) and the generator in a pre-trained PI-GANs are employed as the surrogate for $u$ in these two methods, respectively. Further, both the sampling or variational inference approaches can be utilized for obtaining the posterior samples for $\theta$. In addition to the Bayesian methods, the Monte Carlo dropout \cite{gal2016dropout} (MCD) as well as the deep ensemble \cite{lakshminarayanan2017simple} (DEns) which employ the standard NN as surrogates for $u$ and/or $\lambda$ can be combined with PINNs to quantify uncertainties in problems with known physics \cite{zhang2019quantifying,psaros2022uncertainty}. In \cite{psaros2022uncertainty}, the B-PINNs, MCD- and DEns-based PINNs are referred to as U-PINNs, and the PI-GAN-based functional prior method is referred to as PI-GAN-FP, respectively.

% For physics informed learning, one of the most well-known methods is B-PINN \cite{yang2020bayesian}, which serves as a straightforward adaptation to Bayesian framework of PINN, and a very useful tool to solve PDE problems with noisy data. Hamiltonian Monte Carlo (HMC) \cite{neal2011mcmc} and VI are used for posterior inference over the parameters. {\color{red} B-PINN with HMC is considered as the golden standard for PINN with UQ.} However, \cite{meng2021learning} pointed out that the high dimensionality of B-PINN's parameters leads to expensive computational cost and difficult posterior estimation in the inference stage, and it further proposed the functional prior (FP) method to address this issue, which utilizes generators, e.g. PI-GAN, to first learn from the physics and the historical data, correlates the distribution of data with a tractable distribution in the latent space, e.g. Gaussian, and then perform posterior inference on new, probably unseen dataset. 

% Both B-PINN and FP mentioned above are considered as methods in the family of Bayesian inference. As opposite, many UQ methods from the deterministic framework have been developed in recent years \cite{abdar2021review}, only a few of which, however, have been utilized for physics informed learning. Dropout, as one of the most popular regularization methods as well as a UQ method \cite{gal2016dropout}, was first used to quantify uncertainty in PINN by \cite{zhang2019quantifying}. In \cite{psaros2022uncertainty}, deep ensemble \cite{lakshminarayanan2017simple} was tested as a UQ method for PINN as well as DeepONet.


% For physics agnostic learning, DeepONet is of high importance. On one hand, as mentioned above, equipped with deep ensemble, DeepONet itself could be viewed as a physics agnostic UQ method; on the other hand, a trained DeepONet could also serve as a PDE-agnostic function and connects to other approximator, e.g. an NN. FP could also be viewed as a physics-agnostic UQ method, as long as the training of its generator as well as its inference are performed with no physics.

% For the special case of learning neural operators described in Section~\ref{sec:uqINsciml:sciml}, the solution $u$ is modeled with a DeepONet surrogate parametrized by $\theta$ and posterior inference is performed as above. 
% This model is referred to as U-DeepONet in \cite{psaros2022uncertainty}.
% However, for the more general case in which the inference input data are noisy, the DeepONet is pre-trained with fixed parameters, and the input $f$ is modeled with a BNN or a GAN-FP, denoted by $\cM$ in Fig.~\ref{fig:neurals}.
% These models are referred to as PA-BNN-FP and PA-GAN-FP, respectively, in \cite{psaros2022uncertainty}. 
% Posterior inference is performed as above for the BNN parameters $\theta$ or the GAN input $\theta$. 


For physics agnostic learning, a DeepONet parameterized by $\theta$ is employed as the surrogate for the solution $u$. Different ways have been developed for the uncertainty quantification in DeepONet. In the Bayesian framework, \cite{lin2021accelerated} proposed to employ the BNNs in DeepONet and a sampling method is then utilized to obtain the posterior samples for the parameters in BNNs. As for deterministic methods, extensions of the standard training of DeepONets like deep ensembles are used for quantifying uncertainties in predictions \cite{psaros2022uncertainty,yang2022scalable}. The approach in \cite{lin2021accelerated} can address both the epistemic and aleatoric uncertainties, while the ones in \cite{psaros2022uncertainty,yang2022scalable} is only able to quantify the epistemic uncertainty.  Further, the inference input $f$ should be represented in the same way as used in the training, i.e., the number of the discrete values as well as their locations. For a more general case in which the inference input and/or output data are noisy and are measured at a certain number of random locations,  \cite{meng2021learning} proposed to combine a pre-trained DeepONet and a generative adversarial network (GAN) based functional prior to quantify the uncertainties in predictions. In \cite{psaros2022uncertainty}, the BNNs are utilized as an alternative to the GANs in \cite{meng2021learning}. These two methods are referred to as PA-GAN-FP and PA-BNN-FP in \cite{psaros2022uncertainty}, respectively.  
%These models are referred to as PA-BNN-FP and PA-GAN-FP, respectively, in \cite{psaros2022uncertainty}. 
%Posterior inference is performed as above for the BNN parameters $\theta$ or the GAN input $\theta$. 


% DeepONet, equipped with deep ensemble, is capable of quantifying the model uncertainties. as a physics agnostic UQ method; on the other hand, a trained DeepONet could also serve as a PDE-agnostic function and connects to other approximator, e.g. an NN. FP could also be viewed as a physics-agnostic UQ method, as long as the training of its generator as well as its inference are performed with no physics.

%For neural ODEs/PDEs, the solution $u$ is modeled with a \textit{surrogate} parametrized by $\theta$ and denoted by $\cM$ in Fig.~\ref{fig:neurals}.  
%In \cite{psaros2022uncertainty}, these models are referred to as U-PINN, and PI-GAN-FP, respectively. 
%In all cases, different $\theta$ values correspond to different functions $u_{\theta}$. 
%We refer to the surrogate combined with a probability distribution $p(\theta)$ for $\theta$ as a \textit{process}. 
%As mentioned earlier in the paper, posterior inference obtains representative $\theta$ samples that explain the data $\cD$, based on the process definition.
%Also, the problem parameters $\lambda$ can either be unknown constants or unknown fields depending on the problem setup.  
%In such cases, we can use surrogates for $\lambda$, parametrized by $\theta_{\lambda}$. 
%Accordingly, posterior inference is performed for both $\theta$ and $\theta_{\lambda}$ simultaneously.

%For the special case of learning neural operators described in Section~\ref{sec:uqINsciml:sciml}, the solution $u$ is modeled with a DeepONet surrogate parametrized by $\theta$ and posterior inference is performed as above. 
%This model is referred to as U-DeepONet in \cite{psaros2022uncertainty}.
%However, for the more general case in which the inference input data are noisy, the DeepONet is pre-trained with fixed parameters, and the input $f$ is modeled with a BNN or a GAN-FP, denoted by $\cM$ in Fig.~\ref{fig:neurals}.
%These models are referred to as PA-BNN-FP and PA-GAN-FP, respectively, in \cite{psaros2022uncertainty}. 
%Posterior inference is performed as above for the BNN parameters $\theta$ or the GAN input $\theta$. 

% In passing, note that the ensemble posterior inference methods, summarized in Table~\ref{tab:uqt:over}, do not require a prior $p(\theta)$ and thus, we only need to define the surrogate component.

% \subsubsection{Likelihoods}\label{sec:likelihoods}

% Given a set of paired noisy observations $\cD = \{x_i,u_i\}_{i=1}^{N}$, our goal is to construct a distribution $p(u|x, \cD)$ for predicting the value of $u$ at any new location $x$. 
% For each $x$, it is commonly assumed that $u(x)$ produced by the data-generating process contains both a deterministic part $u_c(x)$ as well as some additive noise $\epsilon_u$, i.e., $u(x) = u_c(x) + \epsilon_u$.
% This noise is typically called data or aleatoric uncertainty. 
% For modeling this process, we assume a \textit{likelihood function} denoted by $p(u|x, \theta)$, with parameters $\theta=[\theta_1,\dots,\theta_K]^T$ to be inferred from the available data.
% Further, for defining $p(u|x, \theta)$ we construct a model $u_{\theta}(x)$ that captures the deterministic part of $u(x)$ at some location $x$ and assume a model for the noise.
% For example, the factorized Gaussian likelihood function, given as
% \begin{equation}\label{eq:uqt:pre:bma:Glike}
% 	p(u|x, \theta) = \cN(u|u_{\theta}(x), diag(\Sigma_{u}^2)) = \prod_{d = 1}^{D_u}\frac{1}{\sqrt{2\pi \sigma_{u}^2}}\exp(-\frac{(u_d-u_{\theta}(x)_d)^2}{2\sigma_{u}^2}), 
% \end{equation}
% with the subscript $d$ denoting each of the $D_u$ dimensions of $u$, is often used for multi-dimensional function approximation problems.
% In Eq.~\eqref{eq:uqt:pre:bma:Glike}, the output vector $u_{\theta}(x)$ is the mean of the Gaussian distribution assumed for $u$ at location $x$, $diag(\Sigma_{u}^2)$ is a diagonal covariance matrix with $\Sigma_{u}^2 = [\sigma_{u}^2,\dots,\sigma_{u}^2]$ in the diagonal, and $\sigma_{u}^2$ may either be known or assumed, or inferred from data.

% For neural ODEs/PDEs, the observations in the dataset $\cD = \{\cD_f, \cD_b, \cD_u, \cD_{\lambda}\}$ are typically obtained with a data acquisition device and are noisy. 
% In this regard, we employ four likelihood functions for approximating the $f, b, u$ and $\lambda$ distributions, denoted as $p(f|x, \theta), p(b|x, \theta), p(u|x, \theta)$, and $p(\lambda|x, \theta)$, respectively.
% The total likelihood of the dataset $\cD$ becomes
% \begin{equation}\label{eq:uqt:pre:pinn:like}
% 	p(\cD|\theta) = p(\cD_f|\theta)p(\cD_b|\theta)p(\cD_{u}|\theta)p(\cD_{\lambda}|\theta),
% \end{equation}
% where 
% \begin{equation}
% \begin{aligned}\label{eq:uqt:pre:pinn:likes}
% 	p(\cD_f|\theta) & = \prod_{i=1}^{N_f}p(f_i|x_i, \theta) \text{; } & p(\cD_b|\theta) & = \prod_{i=1}^{N_b}p(b_i|x_i, \theta);\\
% 	p(\cD_u|\theta) & = \prod_{i=1}^{N_u}p(u_i|x_i, \theta) \text{; } & p(\cD_{\lambda}|\theta) & = \prod_{i=1}^{N_{\lambda}}p(\lambda_i|x_i, \theta).
% \end{aligned}
% \end{equation}

% For neural operators, we assume that $f$ and $b$ in Eq.~\eqref{eq:intro:piml:pinn:pde} are known and the dataset $\cD_{\lambda}$ consists of clean data.
% Nevertheless, $\cD_u$ consists of noisy data in general.
% In this regard, a likelihood function is employed for the $u$ data, denoted by $p(u|x, \xi, \theta)$, and the total likelihood is given as
% \begin{equation}\label{eq:uqt:pre:don:like}
%     p(\cD|\theta) =\prod_{i=1}^{N}\prod_{j=1}^{N_u}p(u_j^{(i)}|x_j^{(i)}, \xi_i, \theta). 
% \end{equation}

% \subsubsection{Posterior inference}\label{sec:inference}

% Performing UQ for neural ODEs/PDEs and operators involves combining the constructed model with a posterior inference method. 
% In this section, we provide a summary of the considered inferences for producing surrogate parameter $\theta$ samples and subsequently, the sought function samples.

% Obtaining the posterior distribution of $\theta$ is computationally and analytically intractable. 
% To address this issue, approximate inference aims to approximate the posterior by another distribution and/or obtaining  NN parameter posterior samples $\{\hat{\theta}_j\}_{j=1}^M$ from the posterior.
% In Table~\ref{tab:uqt:over} we provide an overview of the most commonly used methods for obtaining $\{\hat{\theta}_j\}_{j=1}^M$; see Fig.~\ref{tab:uqt:over} and \cite{psaros2022uncertainty} for more details.
% We refer to the HMC, LD, MFVI, and LA methods as \textit{Bayesian}, because they are related with the Bayesian paradigm of obtaining posterior samples, and to the MCD, DEns, SEns, and SWAG methods as \textit{deterministic}, because they can be interpreted as extensions of standard, i.e, deterministic, training of NNs.

% In the package, the default option is to combine the methods with a Bayesian neural network, as a surrogate.
% Alternatively, a GAN functional prior can be used.

%\textcolor{blue}{
%UQ4SciML supports three different types of posterior estimation methods, i.e., sampling-based method, vi-based method, and . Specifically, the sampling- and vi-based posterior estimations are for \textit{Bayesian} methods, and the .  MCMC-based methods utilize Markov chain Monte Carlo to sample directly against, probably un-normalized, posterior distribution. We describe MCMC-based methods as sampling methods. Ensemble-based methods execute standard training of NNs, throughout which samples are collected to group an ensemble. We describe such methods as sampling-through-optimization ones. Finally, VI-based methods are closely related with variational inferences, where posterior is approximated by optimizing some distance, e.g. KL-divergence, between the real one and a parameterized one. After the optimization completes, samples are obtained by sampling against the trained parameterized distribution, and hence we describe such methods as optimizing-and-sampling ones. Types of inference methods should be consistent with the type of model, e.g. an MCMC-based method can not work with a variational inference model, even though they both belong to the family of Bayesian inference.
%}

% \subsubsection{From parameter to function samples}\label{sec:fsamples}

Following approximate posterior inference, the posterior samples for $\theta$ are used for obtaining the statistics of the function samples.
In this regard, the value of $u$ at a location $x$ given the data $\cD$ is a random variable denoted by $(u|x, \cD)$.
The mean of $(u|x, \cD)$ is denoted by $\hat{u}(x) = \mathbb{E}[u|x, \cD]$ and approximated by $\bar{\mu}(x)$ as
\begin{equation}\label{eq:uqt:pre:mcestmc:mean}
	\hat{u}(x) \approx \bar{\mu}(x) = \frac{1}{M}\sum_{j=1}^Mu_{\hat{\theta}_j}(x),
\end{equation}
where $\{u_{\hat{\theta}_j}(x)\}_{j=1}^M$ is the set of NN predictions corresponding to the samples $\{\hat{\theta}_j\}_{j=1}^M$.
Further, the diagonal part of the covariance matrix of $(u|x, \cD)$ is given by
\begin{equation}\label{eq:uqt:pre:mcestmc:totvar}
	Var(u|x, \cD) \approx \bar{\sigma}^2(x) =  \underbrace{\Sigma_{u}^2}_{\bar{\sigma}_a^2(x)}  + \underbrace{\frac{1}{M}\sum_{j=1}^M(u_{\hat{\theta}_j}(x)-\bar{\mu}(x))^2}_{\bar{\sigma}_e^2(x)}. 
\end{equation} 
In this equation, $\bar{\sigma}^2(x)$ represents the approximate total uncertainty of $(u|x, \cD)$, while $\bar{\sigma}_a^2(x)$ and $\bar{\sigma}_e^2(x)$ denote the aleatoric and the epistemic parts of the total uncertainty, respectively.
In practice, a Gaussian (or, e.g., a Student-t) distribution is commonly fitted to the posterior samples.
For example, we denote as $\pazocal{N}(\bar{\mu}(x), \bar{\sigma}^2(x))$ the Gaussian approximation to the samples $\{u_{\hat{\theta}_j}(x)\}_{j=1}^M$ at an arbitrary location $x$, where $\bar{\mu}(x)$ and $\bar{\sigma}^2(x)$ are obtained via Eqs.~\eqref{eq:uqt:pre:mcestmc:mean} and \eqref{eq:uqt:pre:mcestmc:totvar}, respectively.

\subsection{Performance evaluation and post-training calibration}\label{sec:calibration}


\begin{table}[h]
	\centering
	\footnotesize
	\begin{tabular}{clc}
		\toprule
		\multicolumn{3}{c}{\textbf{Post-training calibration methods}}\\
		\midrule
		Reference & Short description & Name in library
		\\
		\midrule
		\multirow{2}{*}{\cite{levi2019evaluating}}  &  Re-weighting optimally all predicted variances. & \multirow{2}{*}{\textbf{\texttt{calibration.var}}} \\
		 & Modifies only the variance of the predictions. & \\
		\arrayrulecolor{black!30}\midrule
		\multirow{3}{*}{\cite{kuleshov2018accurate}} &  Approximates misscalibration function & \textbf{\texttt{calibration.cdf}}
		\\ & and applies it to all predictive distributions. & (not currently
         \\ & Modifies both the mean and the variance of all predictions. & implemented)\\
		\arrayrulecolor{black!30}\midrule
		\multirow{3}{*}{\cite{zelikman2020crude}} & An empirical distribution is fitted to the scaled residuals & \textbf{\texttt{calibration.crude}}
		\\ & that correspond to the calibration dataset.& (not currently
		\\& Modifies both the mean and the variance of all predictions.& implemented) \\ 
		\arrayrulecolor{black}
		\bottomrule
	\end{tabular}
	\caption{Overview of the post-training calibration methods considered in this paper. 
	These methods can be used for improving statistical consistency; i.e., how closely the predictive model matches the data-generating distribution.
    To that end, an additional dataset $\cD_r = \{x_i, u_i\}_{i=1}^{N_r}$ is required after training.
    This can be a left-out calibration dataset, similar to validation and test sets.
	}
	\label{tab:calibration}
\end{table}

Performance evaluation is necessary for model
selection, e.g., prior/architecture optimization, comparison between UQ methods, and overall quality evaluation of the UQ design procedure.
As reviewed in \cite{psaros2022uncertainty}, performance evaluation metrics include the relative $\ell_2$ error for evaluating accuracy, the mean predictive likelihood for evaluating predictive capacity, and the root mean squared calibration error for evaluating statistical consistency; i.e., how closely the predictive model matches the data-generating distribution.


Further, for improving statistical consistency, we provide in Table~\ref{tab:calibration} three post-training calibration approaches.
To use these approaches an additional dataset $\cD_r = \{x_i, u_i\}_{i=1}^{N_r}$ is required after training.
This can be a left-out calibration dataset, similar to validation and test sets.
